Comparison of STR and EMLSR Performance in Wi-Fi 7 MLO

This project compares the performance of simultaneous transmit and receive (STR) and enhanced multi-link single radio (EMLSR) within Multi-Link Operation (MLO) in Wi-Fi 7 networks. Using the ns-3 simulator, we evaluate both techniques under various scenarios, including changes in modulation coding scheme (MCS), bandwidth, link quality, and interference levels. Key performance metrics such as latency, throughput, and energy efficiency are analyzed to determine the trade-offs between STR and EMLSR. The results demonstrate that STR achieves higher throughput and lower latency due to dual-link utilization, making it suitable for high-load environments. In contrast, EMLSR balances energy efficiency with responsiveness, making it advantageous for power-sensitive applications. This analysis provides insights into the strengths and limitations of STR and EMLSR, guiding optimal deployment strategies for future Wi-Fi 7 networks.

==> acronyms.tex <==
\begin{acronym}
    \acro{AP}{access point}
    \acro{BW}{bandwidth}
    \acro{EHT}{extremely high throughput}
    \acro{EMLSR}{enhanced multi-link single radio}
    \acro{MCS}{modulation coding scheme}
    \acro{MLD}{multi-link device}
    \acro{MLO}{Multi-Link Operation}
    \acro{QAM}{quadrature amplitude modulation}
    \acro{QPSK}{quadrature phase-shift keying}
    \acro{SLD}{single link device}
    \acro{SLO}{Single-Link Operation}
    \acro{STA}{station}
    \acro{STR}{simultaneous transmit and receive}
\end{acronym}
